COPSS-lite: Lightweight ICN Based Pub/Sub for IoT Environments

Information Centric Networking is a new networking paradigm that treats content as first class entity. It provides content to users without regards to the current location of the content. The publish/subscribe systems have gained popularity in Internet. Pub/sub systems dismisses the need for users to request every content of their interest. Instead, the content is supplied to interested users (subscribers) as and when it is published. CCN/NDN are popular ICN proposals widely accepted in the ICN community however, they do not provide an efficient pub/sub mechanism. COPSS enhances CCN/NDN with an efficient pub/sub capability. Internet of Things (IoT) is a growing topic of interest in both Academia and Industry. The current designs for IoT relies on IP. However, the IoT devices are constrained in their available resources and IP is heavy for their operation.We observed that IoT's are information centric in nature and hence ICN is a more suitable candidate to support IoT environments. Although NDN and COPSS work well for the Internet, their current full fledged implementations cannot be used by the resource constrained IoT devices. CCN-lite is a light weight, inter-operable version of the CCNx protocol for supporting the IoT devices. However, CCN-lite like its ancestors lacks the support for an efficient pub/sub mechanism. In this paper, we developed COPSS-lite, an efficient and light weight implementation of pub/sub for IoT. COPSS-lite is developed to enhance CCN-lite and also support multi-hop connection by incorporating the famous RPL protocol for low power and lossy networks. We provide a preliminary evaluation to show proof of operability with real world sensor devices in IoT lab. Our results show that COPSS-lite is compact, operates on all platforms that support CCN-lite and we observe significant performance benefits with COPSS-lite in IoT environments.

==> copss_architecture.tex <==
\hide{\begin{figure}[t!]
\centering
  \includegraphics[width=1.0\linewidth]{figures/NDN_Architecture_with_COPSS.pdf}
%\vspace{-3mm}
  \caption{CCN Forwarding Engine Model\cite{NDN} with COPSS\cite{COPSS} Subscription Table}
  \label{fig-ndn_copss_data_structure}
% \vspace{-6mm}
\end{figure}
}
COPSS drew special attention to the popular pub/sub systems running over IP in the Internet.
It described how the current pub/sub systems in Internet are supported mainly via the client side applications and servers to deliver the published content to subscribers.
COPSS showed the additional responsibility/burden that is incurred with the IP based solutions.
In\cite{Multicache,Corona} authors show the IP based solutions tend to waste network resources.
Hence a Content-Oriented Pub/Sub System (COPSS) was proposed to enhance the initial design of CCN by integrating it with an efficient and scalable pub/sub capability.
In essence, COPSS enhanced the pull based model of CCN by incorporating a push based model with multicast capability at the content-centric layer to support pub/sub systems in CCN.

COPSS based its pub/sub architecture on utilizing the concept of Content Descriptors (CD). In general, CD's are some features of the content like keywords, date of publication, identity of the publisher, \etc
Further, COPSS expanded the scope of CD's to support ontologies, content hierarchies and context based content identification.
COPSS also identified a problem with NDN to support pub/sub: NDN requires the subscribers to either know the publisher or the precise name of the content published.
Since, this is not a mandatory requirement in pub/sub environment as it is desired to eliminate temporal dependency, NDN fails to support this need.
The COPSS architecture uses multicast at the content-centric layer.
Similar to PIM-SM (\cite{PIM-SM}) COPSS also uses multiple-senders and multiple-receivers with multicast capability along with Rendezvous Point (RP).

Figure\ref{fig-ndn_copss_data_structure} shows the COPSS architecture. % with CCN forwarding engine.
COPSS adds a Subscription Table to the initial CCN forwarding engine.
Every COPSS router maintains the subscription table for enabling pub/sub in a distributed and aggregated manner.
COPSS also introduces two new packets: \emph{Subscribe} and \emph{Publish}.
The Subscribe packet is used by the users to subscribe to a certain CD while the Publish packet will be used by the publisher to publish content for a single or group of CD's \ie a piece of content can be associated with multiple CD's.
%Each piece of content is associate with CD's defined by the publishers.
Each CD is assigned to a respective RP node in the network.
%The CCN network assigns each CD to RP.
Subscribers will subscribe to the content of their interest by subscribing to the associated CD's, resulting in a join.
When a router receives a subscription request, it will add an entry in its Subscription Table with the CD and the incoming face of the request and forward the request upstream.
The subscription request is forwarded towards RP with each intermediate router adding an entry for the subscription. % request.
When the publisher generates any content, he associates the content with the CD's.
Whenever the content is published, it travels along the multicast tree towards the responsible RP.
When a router receives a publication packet, it checks the subscription table for any one of the CD's in the publication.
If a match is found then the router forwards the publication along the matched interfaces.
However, only a single copy of the publication is forwarded on each interface, irrespective of the number of subscribers downstream. This avoids, unnecessary traffic and duplicate/multiple copies delivered to the subscribers of more than one CD in the publication.

COPSS also provides a two-step communication process which allows the publisher to exercise control over the access and policy of the published contents. In a two-step communication process, the publishers generate a snippet of the original content with the associated CD's and send it to subscribers. Interested subscribers can then use these CD's to subscribe to the full-length original content. The publishers then publish the original content which is forwarded to the interested subscribers as explained previously.













